On Difficulties of Cross-Lingual Transfer with Order Differences: A Case Study on Dependency Parsing

Different languages might have different word orders. In this paper, we investigate cross-lingual transfer and posit that an order-agnostic model will perform better when transferring to distant foreign languages. To test our hypothesis, we train dependency parsers on an English corpus and evaluate their transfer performance on 30 other languages. Specifically, we compare encoders and decoders based on Recurrent Neural Networks (RNNs) and modified self-attentive architectures. The former relies on sequential information while the latter is more flexible at modeling word order. Rigorous experiments and detailed analysis shows that RNN-based architectures transfer well to languages that are close to English, while self-attentive models have better overall cross-lingual transferability and perform especially well on distant languages.

==> previous/introduction.tex <==
\section{Introduction}
\NoteNP{Do literature survey on multi-lingual transfer (for different tasks not only parser).}

% \todo{Motivate the importance of transfer learning for cross-lingual tasks.}
\NoteNP{You can probably learn some motivations from this paper: \url{http://nakashole.com/papers/2018-emnlp-norm.pdf}}
%The usage of deep neural networks require a large amount of annotated data which is expensive to manage for domains like natural language processing (NLP) that require expert annotators.
Many NLP tasks have achieved high accuracy in resource rich languages (e.g., English, Chinese) thanks to the availability of large-scale datasets.
%On the other hand, building models utilizing neural networks is still a challenging task for low resource languages (Japanese, Swahili).
However, it is still a challenging task to learn models for low resource languages because of a lack of rich annotated data.
To subsidize the requirement of large-scale annotations for such languages, cross-lingual transfer has become a motivation for a variety of NLP tasks \cite{zhou2016transfer, guo2015cross}. 
\NoteKW{It's a bit weird to say the reason we want to transfer is due to lack of data -- people can argue this zero-shot setting is unrealistic as we do have a few annotated data in all language. It's probably better to ask a higher-level research question rather from an engineering aspect.}

Cross-lingual transfer has achieved remarkable performances by learning multilingual word embeddings that map words from different languages into the same embedding space. These low-dimensional representations are then used as inputs to neural networks to bridge languages. However, the underneath challenges for transferring from one language (source) to another (target) not only include vocabulary and lexical semantics, but also other language differences such as word order and syntax.
The difficulty of cross-lingual transfer depends on the distance between the source and the target language.
For example, transferring language specific information from English to Japanese is hard since they are distant languages \cite{chiswick2005linguistic}.\newcite{} have shown that sharing higher level representations, such as a Recurrent Neural Networks (RNNs) could sometimes hurt the transferability. 

% \todo{What are the challenges for transferring dependency parser systems?}
% French, Dutch languages are closer to English and Japanese, Chinese are some of the distant languages.
% The major challenge in transferring a parsing system from one language to another is the lexical features, e.g. words, which are not directly transferable across languages.
An effective transferable model across languages is expected to learn language invariant features when trained on the source language. 
When a recurrent neural networks (RNNs) is the central component in the transfer model, we expect the RNNs to learn features that are less susceptible to specific language and are transferable across languages.
In this work, we show that RNNs are not a robust transferable language encoder since it relies too much on the word order information, and thus cannot transfer well between languages that have distinct word order.
We propose to use relation-aware multi-head self-attention architecture \cite{shaw2018self} in contrast to RNNs to capture context information, and we show that the self-attention mechanism transfers better across languages even when the target languages are distant from the source language.

% \todo{Motivate the usage of self-attention mechanism and relative position encodings.}

The multi-head self-attention was first proposed in Transformer \cite{vaswani2017attention} which has shown improvements in a variety of NLP tasks, e.g., machine translation (cite a paper), constituency parsing \cite{kitaev2018constituency} and also demonstrated strong language understanding \cite{devlin2018bert} that are transferable on a wide variety of NLP tasks.
A recent work \cite{lakew2018comparison} showed that the self-attentive model offers significant advantages over RNN-based models on multilingual machine translation task.
\NoteKW{This paragraph is weak -- we will need to elaborate our motivations rather than just citing a few papers says self-attention has been also used in other places. In general, need to think carefully how to structure the introduction. Currently, it looks like we blindly borrow this and borrow that from other papers and put them together to hope things work. Instead, we should structure the introduction in a motivation-driven. Discuss what would be the challnege to do multi-lingual transfer and then say, our solution are the combination of all these components.}

By taking this as a motivation, we study the cross-lingual transferability of the enhanced relation-aware self-attentive encoder proposed in \cite{shaw2018self}.
Relation-aware self-attention makes an effective use of relative positions, or distances between sequence elements and can decide which information can be transferred between different locations in the sentence and we hypothesize that this characteristics makes the self-attentive encoder transferable across different families of languages.


% Self-attentive encoders have shown to perform better than RNN-based encoders on a wide variety of tasks

To evaluate our conjecture that relation-aware self-attention architecture is a better language encoder that transfers better, we use dependency parsing task as our testbed.
We chose dependency parsing as the evaluation task, primarily because of the availability of annotated data across a wide spectrum of languages.
Moreover, parsing is considered as one of the low-level NLP tasks \cite{hashimoto2016joint} that highly relies on syntactic structure of languages and thus can reflect the transferability of neural architectures.

% \todo{What has been done previously for multilingual dependency parsing via transfer learning?}
% Previous approaches \cite{AAAI2016} are based on distributed feature representations where symbolic features are mapped to a continuous representation space, that can be shared across languages.


% \todo{How we are different from previous works?}


\todo{A highlight of our findings.}


% Note from Kai-Wei
% Parsing is just one way to show transfer ability of the RNN-free architecture across languages
% different language has different properties
% Encoding part is showing the difference between RNN and transformer
% Decoding part is showing the difference between graph and transition based parsing

% Nanyun
% The ability to transfer across languages is important.
% We posit RNNs are not a good encoder for transfer because it relies too much on word order. -- Word order is a key characteristics for language. Word order differences characterize the distances of languages.
% We propose relation-aware multi-head self-attention architecture to capture context information without relying on word orders, and we show better tranferrability for the languages that are distant.
% We use dependency parser as our testbed because 1) we have vast amount of data across a large spectrum of languages; 2) it is on the bottom level of NLP stack, so it better reflect the transferability; 3) team: feel free to come up with more reasons!!!

% Main story will evolve around - What is the best architecture that can be transferred across language? And dependency parsing is just a test bed.

% Zhisong
% I think we should be careful about describing model, we can say that Transformer relies less than RNN at word ordering, but in fact, word ordering (or simply word context) is still an important information for parsing. Remember that we tried remove positional embedding, and the results get much worse. Thus, I think the main topic is about the degree or flexibility of modeling language ordering information. (We should agree on a consistent saying in the next meeting!!)

% Transfer across language is more sensitive to word order information.


==> previous/method.tex <==
\section{Model}
%\todo{Maybe one of the main theme of this paper can be exploring a good between the power of parsing model and the flexibility for transfer learning? Therefore, when describing model, we may want to remember this theme.}
\NoteZS{I think we can be more brief in this Model part? since most the models are exiting ones.}

% Give an overview of a dependency parsing system.
% Keep cross-lingual transfer is the main theme. 
Learning multilingual transferable feature encoder is one of the fundamental requirements of building cross-lingual NLP models.
The success of cross-lingual transfer largely depends on the multilingual feature encoder that is expected not to rely too much on language specific information.
For example, capturing word-order information precisely of English language by the feature encoder, perhaps help a similar language (ex., Swedish, Dutch) but may cause losing the effectiveness in representing features for a distant language (e.g., Hebrew, Indonesian).
In section \ref{sec:mul_feat_enc}, we briefly discuss our experimental multilingual feature encoding techniques investigated in the context of multilingual dependency parsing.

Dependency parsing paradigms are broadly categorized into graph-based and transition-based parsers \cite{chiswick2005linguistic}.
In this work, we aim to study the transferability of both type of parsing techniques and we discuss our experimental models in section \ref{sec:dec_dep_parse}.
% we briefly describe the three major components for multilingual dependency parsing, (1) multilingual lexicon representation, (2) multilingual feature encoders, and (3) decoders.

\subsection{Multilingual Feature Encoders}
\label{sec:mul_feat_enc}

\subsubsection{Lexicon Representation}
% why we are using multilingual embedding? motivate it.
Transferring NLP models across languages in (1) \textit{zero-shot setting}, when no
supervision is available, and in (2) \textit{low-resource setting}, when small amount of
supervision is available in the target language has largely relied on multilingual lexicon representation.
Recent works in  neural machine translation \cite{gu2018universal}, cross-lingual entity linking \cite{upadhyay2018joint}, multilingual dependency parsing \cite{guo2015cross, guo2016representation} considered bilingual or multilingual word embeddings as the basic lexical feature representations. 
In this work, we use fasttext vectors \cite{bojanowski2017enriching} as the monolingual word representations which are later mapped into a common space following the offline transformation method proposed in \cite{smith2017offline} to get multilingual word vector representations.
% \NoteZS{In fact, we are now using \cite{smith2017offline}'s method for embedding projection, I've also described this in Section 5.1.Settings.}
\NoteKW{Some of things you wrote here should go to related work section. Put only things relevant to our modeling. Need to elaborate more besides just citing a few papers -- you don't need to put great details, but also you cannot assume readers will go to those references to understand what you're talking about. }

\subsubsection{Learning Context Representations}
Learning context representation refers to estimating a parameterized function that maps a sequence of $n$ input vector representations $x_{1:n}, x_i \in R^{d_{in}}$ to a sequence of $n$ output vectors $h_{1:n}, h_i \in R^{d_{out}}$.
For the dependency parsing task, the input vectors usually embed information of the word-identity, and part-of-speech (POS) tag.
With the growth of deep learning, recurrent neural networks (RNNs) has become the primary choice to learn a parameterized function for modeling sequential data.
Although RNNs are good at capturing sequential information, its inherent sequential nature prohibits parallel computation within training examples.
To get rid of this limitation, a multi-head self-attention based architecture is proposed in \cite{vaswani2017attention} that demonstrated superior performance in a variety of NLP tasks.   
However, it is still unclear that how effective the RNN or self-attention based encoders are in cross-lingual transfer.
We will show in section \ref{sec:results}, while RNN based encoder transfers better to the target languages that are closer to the source language but self-attention based encoder generalizes better across languages that are distant from the source language. 
Below we briefly describe the two encoder prototypes that we study in this work.

\NoteKW{Here, you want to emphasize despite these dependency parsing algorithms and architectures have been studied, it is unclear how they can transfer information from one language to the other. Besides simply describe the architecture, the important part is to discuss how these encoder/decoder capture information and put them in the context of cross-lingual transfer. }


\paragraph{Sequence encoder}
We use a $k$-layer bidirectional RNN following \cite{kiperwasser2016simple} as the sequence encoder.
More specifically, we employ a 3-layers bidirectional LSTM \cite{hochreiter1997long} on top of the input vectors to provided contextualized vectors.
% \NoteZS{This should correspond to \cite{dozat2017biaffiine} or earlier TACL 16: Q16-1023}

\paragraph{Self-attentive encoder}
We adopt the multi-head self-attention encoder from the Transformer architecture proposed in \cite{vaswani2017attention}.
We use the terms ``self-attentive encoder'' and ``Transformer encoder'' interchangeably throughout the paper.
In the Transformer encoder, sublayers are consists of a mult-head attention mechanism followed by a parameterized linear transformation to produce the output vectors.
In particular, each head in multi-head attention takes the sequence of input vectors and computes a new sequence of vectors of the same length.
The resulting vectors from each head are concatenated and transformed using a feed-forward network which is feed to the next sublayer.
A residual connection is employed in each sublayer that helps to propagate information from lower layers to higher layers.  
% followed by a layer normalization.
% So, in essence, a self-attentive encoder composed of $n$ identical sublayers stacked on top of each other.
% where each can be views as a function, $F = LayerNorm(x + Sublayer(x))$.

To capture sequence information, positional embeddings are added to the input vectors before feeding them into the encoder.
Unlike sequence (RNNs) encoders Transformer encoder does not have any recurrence and thus the additional position encodings in the input representations has become a requisite to model sequence data.
However, the absolute position embeddings used in \cite{vaswani2017attention} loosely embed the direction and distance information among the input elements.
In order to model the pairwise relationships between input elements, \cite{shaw2018self} proposed a relation-aware self-attention mechanism.
In contrast to absolute position encodings, \cite{shaw2018self} suggested to model the relative position differences between input elements.

In dependency parsing, the distance information between the input elements is crucial.
For example, the information that whether the head word is in the left or right of the modifier can be utilized by one of the attention heads. 
Also, the distance between the head word and the modifier for specific dependency types can be used by other attention heads.
We show in section \ref{sec:pos_rep_trans} that the average improvement is significant when relative position encodings are used in conjunction with the transformer encoder. 
However since we aim to build transferable parser across languages, we do not want the encoder highly depend on the direction information.
For example, a parser trained on ``SVO'' (ex., English, French) languages may not generalize well on ``VSO'' (e.g., Arabic, Hebrew) languages.
To let the encoder be flexible on this language property, we consider the absolute relative distances between the input elements.
So, in contrast to modeling the input as a labeled,
directed, fully-connected graph as proposed in \cite{shaw2018self}, we assume the edges in the graph are undirected. 
% The average improvement is 1.5\% in terms of UAS over 31 languages when relative absolute distance features are incorporated with the Transformer.
We enhance the OpenNMT \cite{opennmt} Transformer implementation\footnote{https://github.com/OpenNMT/OpenNMT-py/blob/master/onmt/encoders/transformer.py} with relation-aware positional embeddings.

\subsection{Decoders for Dependency Parsing}
\label{sec:dec_dep_parse}
% Graph based decoder do not use RNN but stakcPtr model does, so we can motivate the usage of RNN-free decoder for cross-lingual transfer.

% Talk about language similarities first.
The success of transferring a dependency parser in other languages depends on the decoding algorithm which should be robust to the word ordering conventions of languages.
In this work, we study the two dominant categories of dependency parsing, (1) the local and greedy transition-based method, and (2) the globally optimized
graph-based approach in cross-lingual transfer setting.
In transition-based parsing, the objective is to learn a sequence of actions that produce the correct parse tree. 
On the other hand, in graph-based parsing, the goal is to learn a scoring function over all possible dependency trees such that the correct tree is scored above all the other trees.
Both the approaches have their strength and weaknesses for transfer learning which we briefly describe next.
% In this paper, we study both types of parsing methods combined with two different feature encoding techniques.

% Both graph and transition based parser doesn't rely on word order. So, it should be invariant of language order.
% Transition based parser has error propagation issue. Although beam search can subsidize.
% Graph based parser relies on global information. Specially when languages have different word order, the model may makes mistake on initial dependency arcs decision.
% Not to rely too much on word order, we ignore directional information.

% \noindent\smallskip
% \textbf{Transition-based decoder}
\paragraph{Transition-based decoder}
The principle notion of transition-based algorithms is constructing a parse tree by processing the input sentence sequentially (in general, from left to right).
Although transition-based parsers are efficient in terms of time complexity, they suffer from error propagation \cite{mcdonald2011analyzing} because of making decision at each step by looking into the local information.
However, recently \cite{ma2018stack} proposed \emph{stack pointer networks} (StackPtr), a transition-based architecture for dependency parsing that conserves the global view of the sentence to solve the error propagation issue.
Technically, the StackPtr parser acts incrementally, in a top-down and deep-first fashion.
At each decoding step, StackPtr selects a child for the current head word by pointing to one of the input elements.
The selection process of the child depends on the attention scores between the contextualized vectors of the input elements produced by the encoder and a decoder state representation for the current head word.
% StackPtr employs RNNs as the encoder and decoder.

We posit that an effective transferable decoding method requires to look into the global view of the input sentence at each time step, so that irrespective of the word order of a language, it can choose the correct dependent for the head words. 
Therefore, we select the StackPtr decoder to study its' cross-lingual transfer ability. 
\NoteWA{Not sure how to write a conclusive sentence here.}

% \smallskip
% \noindent\textbf{Graph-based decoder}
\paragraph{Graph-based decoder}
The key idea of graph-based parsing is learning a parameterized function that assigns a weight or probability to each possible dependency edges between the input elements and then build a maximum spanning tree (MST) from the weighted edges.
During training, the predicted tree structure is determined by selecting the highest scoring head for each word.
The dependency labels are predicted similarly by using a multi-class MLP which takes a word's and its gold or predicted head word's contextualized vector representation.
In this work, we study the transfer ability of state-of-the-art graph-based Deep Biaffine parser \cite{dozat2017biaffiine}.

Unlike the transition-based approaches, graph-based methods are computationally slow since they perform an exhaustive search over all possible trees.
But due to their principle of finding the globally highest scoring tree, they are better candidate for cross-lingual transfer as we show in section \ref{sec:results}.

% Add discussion on graph-based parsers' effectiveness in transfer learning. Motivate the usage of graph-based parser.



